Position: Stop Anthropomorphizing Intermediate Tokens as Reasoning/Thinking Traces!

Intermediate token generation (ITG), where a model produces output before the solution, has become a standard method to improve the performance of language models on reasoning tasks. These intermediate tokens have been called \say{reasoning traces} or even \say{thinking traces} -- implicitly anthropomorphizing the traces, and implying that these traces resemble steps a human might take when solving a challenging problem, and as such can provide an interpretable window into the operation of the model's thinking process to the end user. In this position paper, we present evidence that this anthropomorphization isn't a harmless metaphor, and instead is quite dangerous -- it confuses the nature of these models and how to use them effectively, and leads to questionable research. We call on the community to avoid such anthropomorphization of intermediate tokens.

==> implications.tex <==
\subsection{Implications}

All together, our counter-intuitive results demonstrate ways in which common interpretations of the intermediate tokens produced by Large Reasoning Models may be anthropomorphizations or simplifications. 
Based on these results, we argue that while the traces certainly seem to help the LLM performance (and may well have mechanistic interpretability \citep{thought-anchors}), intermediate tokens do not have end-user interpretability/semantics and, if the goal is to increase model performance, enforcing trace semantics is unnecessary  and potentially very misleading. 

We note that our position is not that intermediate tokens {\em can't ever have} interpretable meaning but that {\em they don't necessarily have to have} any interpretable meaning. Any human interpretable meaning in the intermediate tokens might be a fortuitous coincidence of such rationales being present in the training data, rather than the model actually doing internal computations corresponding to those statements. In other words, the correlation here may be spurious rather than causal. 
%
This conclusion is also supported to some extent by our companion work with pre-trained models finetuned on Q\&A scenarios \citep{itg-coginterp,bhambri2025interpretable}. 

Our results also raise questions about both the fears of deception in reasoning models based on their chains of thought \citep{alignment-faking}, as well as the earnest pleas to keep chains of thought monitorable for AI safety \citep{korbak2025chain}. 
%
This skepticism seems warranted given that there is no theory drawing causal connections between the semantics of the intermediate tokens and the final solution--beyond the usual ``intermediate tokens change the conditional distribution of the solution tokens." After all, even the proponents of user interpretable semantics for intermediate tokens seem to realize this and write papers talking about why it is incumbent to protect the fragile connection between intermediate tokens and final solutions so as to allow for some kind of monitorability of LLMs (even if it may well be only illusory).
%
Until there is evidence–beyond circumstantial–that LRM reasoning tokens correspond to internal computations, it seems unwise to depend on the intermediate tokens for “safety monitoring” in safety-critical domains. A third-party verification of the solutions/decisions \citep{llm-modulo} seem to be the better way to go in such scenarios.
%

Our results from Section~\ref{sec:length} imply that the prevalent practice of viewing the length of intermediate tokens as a measure of the  computational complexity of the problem instance, might not necessarily be correct. We believe this conflation happened largely because the frontier models charge the end users based on the length of output tokens, a large fraction of which are intermediate tokens in reasoning models.  
%Perhaps intermediate tokens are better seen as the reasoning model's efforts to manipulate it's memory to generate the solution for the current instance starting from the distribution of its own training data (see Figures~\ref{fig:length_v/s_comp} and~\ref{fig:trace_length_scatter}), rather than necessarily a reflection of the computational hardness of the problem instance. 
%
We elaborate on all these concerns and recommendations in a recent position paper \citep{kambhampati2026stop}.

In terms of explaining the role of intermediate tokens in the performance of current reasoning models, our main contribution is to urge the community to look beyond semantics of the reasoning traces, or their correlation to problem complexity. One speculative future direction that we believe merits investigation is viewing intermediate tokens as prompt augmentations \citep{nyas-reasoning}.
The intuition is that for a given task prompt $T$, there may exist an augmentation $\mathrm{PA}$ which boosts the LLM's performance on that task:
\[
\mathbb{P}\bigl(\mathrm{Sol}\bigl(\mathrm{LLM}(T + \mathrm{PA}),\,T\bigr)\bigr)
>
\mathbb{P}\bigl(\mathrm{Sol}(\mathrm{LLM}(T),\,T\bigr)\bigr)
\]
% \raoadd{In terms of explaining the role of intermediate tokens in the performance of current reasoning models, our main contribution is to urge the community to look beyond semantics of the reasoning traces, or their correlation to problem complexity. 
% %why does generating intermediate tokens increase accuracy at all? 
% Our own speculation is that what is helping is finding the right prompt augmentation. That is, for a given task prompt $T$, there exists a prompt augmentation $PA$ which boosts the LLM's performance on that task:}

% \[
% \exists\,PA\;\text{s.t.}\;
% \mathbb{P}\bigl(\mathrm{Sol}\bigl(\mathrm{LLM}(T + PA),\,T\bigr)\bigr)
% >
% \mathbb{P}\bigl(\mathrm{Sol}(\mathrm{LLM}(T),\,T)\bigr)
% \]

Here $\text{Sol}(y,T)$ indicates that $y$ solves $T$, and $\text{LLM}(x)$ is the model’s completion for input $x$. The central challenge then is to learn the Skolem function
\[
\mathrm{PA} = f_{\theta}(T, \text{LLM}),
\]
that maps each task to an effective augmentation. This can be accomplished through modifying the model itself to inherently and automatically augment prompts, as is the case in models that first generate long chains of intermediate tokens before their final answers. Crucially, prompt augmentations have no need to be human‐interpretable. In fact, we see results that back this up in the adversarial prompting literature, where effective jailbreaks can be effected by augmenting prompts with human-uninterpretable strings \citep{zou2023universaltransferableadversarialattacks, cherepanova2024talkingnonsenseprobinglarge, liu2024flipattack, hackett2025bypassingpromptinjectionjailbreak}
 or modifying them with random syntactic permutations, capitalizations, and shufflings \citep{hughes2024best}, \raoadd{as well as the recent work on using intermediate tokens from the continuous latent space \citep{coconut}.}
%
$~$ In this prompt augmentation view, intermediate tokens (and their length) can perhaps be interpreted as the scaffold that the reasoning model uses to learn to manipulate it's %memory 
context to bring the current instance closer to its training distribution,
%generate the solution for the current instance, 
rather than necessarily a reflection of the computational hardness of the problem instance. 

%starting from the distribution of its own training data (see Figures~\ref{fig:length_v/s_comp} and~\ref{fig:trace_length_scatter})


==> sections/01-intro.tex <==
\section{Introduction}

%Introduction: The introduction must state the position, using bold text.

%Alternative Views: The paper can (if appropriate) include an “Alternative Views” section in the main body of the paper (not in an appendix) that describes and addresses one or more viable (not strawmen) positions that are opposed to the paper’s position.

Stop anthropomorphizing intermediate tokens are "thinking"/"reasoning"
traces

Anthropomorphization has been the original sin of AI; drew mcdermott
    LLMs have kicked that into high gear. The most recent example is
    regarding intermediate tokens.. 

Intermediate tokens help, of course

**(The Lack of) Semantics of Intermediate tokens**

Nothing in the way the intermediate tokens are generated and
    "filtered" makes them have any semantics

The intial reasoning traces imitate the training data
     Afterwards, the RL pushes the parameters towards winning
     trajectories--and this global change to the parameters can make it
     even less likely to make sense as reasoning traces

Cite (Rishi hajra work?)

**Seeing Intermediate Token Length as Surrogate for "thinking effort"****

RL part is not doing any miracles--it is not generating new
    reasoning traces! It is just changing parameters ever so little
    towards trajectories that ended up in verified answers.

EXPTS showing 

 [[Stick to ITG for intermediate tokens?]]
    IT vs. ITG (IT can be given or generated.. eventually they become
    generated especially with iterative SFT or RL)
     

The length of intermediate tokens has become a wrong surrogate for
    amount of "reasoning/thinking" the model does--thus leading to
    claims like "RL induces thinking" (when all we mean is that the
    length of intermediate tokens increased). The equally ironic thing
    involve efforts to reduce the length of the intermediate tokens that
    get bandied about as "don't overthink"/"reducing thinking etc"

The length increase of ITG under RL regime can be explained in terms
    of the simplistic MDP model and the simplistic reward
    divvying-up--which incentivize longer chains. The works that then
    claim to produce shorter ones are basically undoing this
    incentivization? (**Can we explain directly with one of those paeprs?**)

  <RL model of LLMs: MDP, Reard divvying]

***What's the harm if people wnat to think of them as having semantics**

Engendering false trust

***WHat is actually happening?**

The Prompt augmentation model

What is happening: Incremental compilation with fixed horizon. 

Overthinking/underthinking etc papers 
%[What are alternate views]


==> sections/02-background.tex <==


\section{Background}
%\subsection{LLMs and LRMs}
%\begin{itemize}
    \item LLMs defined very clearly, there's a looseness to the term, but they're typically used to refer to an actually narrow set of models. Simplicity of their learning procedure, sheer amount of data, and how they surprised us on multiple fronts, even promising advancements on general reasoning tasks.

\item Language is expressive enough to capture, if not the actual underlying reasoning that we do, enough detail about it that we can transfer it from one human to another, and use it as a part of our reasoning processes. This analogy between the linguistically structured tokens output by LLMs and the kinds of things people say when they are "reasoning aloud" has also driven a substantial amount of excitement in research into language models as general-purpose models capable of outputting answers to arbitrary queries, including those that require sound algorithmic execution, symbolic search, or generalizable and novel reasoning. In fact, the opaque nature of these models and our inability to interpret exactly what they are doing "under the hood" to come up with each token.

\item Further work that showed they still were quite limited there... and the particular technique that has been focused on to try to break that barrier.
\end{itemize}
\subsection{Chain of thought}
\begin{itemize}
    \item math domains giving natural CoT outputs, Kojima trick, Wei. These papers drove interest in the field bc: moved past fine-tuning paradigm in Nye, sexier anthropomorphized name, dovetailed into the narrative of emergent abilities with scale

\item connotations that are unwarranted. We use the term for historical reasons. Implications from the connotation are pushing people in the wrong direction: that these chains have interpretable meanings, that they match human cognitive processes (and somehow relate back to Language of Thought hypotheses), that by enhancing their humanness we will get better and more generalizable results

\end{itemize}
\subsection{Defining Intermediate Token Generation}
We define \textit{Intermediate Token Generation} (ITG) as any process in which an LLM first produces a sequence of tokens before outputting the final scored sequence. This can take many forms, from outputting dots, junk tokens, or a special subset of the vocabulary not rendered to the end user to outputting human-looking thoughts or intermediate steps. There are many techniques that induce ITG, which work at anywhere from the prompt level to post-training RL to fine-tuning to even synthetic data generation or natural data selection with an eye towards favoring sequences with a clear separation between questions, shown work, and final answers.

previous work has often assumed, whether implicitly or explicitly, that ITG mirrors human reasoning processes, or has been driven to reproduce human-like derivational traces through ITG. We will argue that this is a flawed approach on two counts: 1) ITG are not directly related to human reasoning processes except through the data that models are trained on and (potentially coincidental) overlap in solutions they learn during training based on the sorts of problems they are post-trained to solve, but the position that these traces have robust semantic content has a significant burden of proof and is often disproven by the content of the traces themselves and 2) it is far from necessary to coerce these traces into human-readable or human-interpretable form let alone into clearly semantically valid form for them to be useful for increasing performance--and that these coercions may be a red herring that actively stifles progress towards both more powerful and more understandable models.
\subsection{Confusing "Useful" and "Correct" ITG}
Forward and backwards directions: 1) and 2). All about the correctness vs utility thing

1) utility => int correctness. Papers that make this unexamined assumption. They only look at the final accuracy, and then don't check. E.g. Kimi, bunch of others?? [CITE]

2) intermediate correctness is necessary for utility. This usually works to inspire directions for work. This claim is actually a lot easier to justify in a certain sense, since there is a grounding of it: an LLM which perfectly outputted only and exactly intermediate token sequences that can be directly mapped onto a specific formal reasoning procedure would provably perform exactly as well as that procedure. However, in practice, this version is violated in multiple important ways. A) ITGs are often only loosely related to some formal procedure (for instance when they are messy human annotations that take inductive leaps and other liberties) B) as mentioned, many papers don't actually check that their methods of inducing ITG, e.g. via SFT, actually generalize robustly in terms of the correctness of the intermediate trace, and C) PRMs introduce additional sources of error in the form of hackable reward models. While *provably* always correct reasoning will always lead to the right answers, it is less clear that *approximately* correct reasoning is particularly effective for neural models that lack the same sorts of structured inductive biases that humans, especially when compared to allowing these models to learn more architecture-appropriate representations and procedures--even though such procedures may be completely uninterpretable to us. The clearest recent example of this is DeepSeek's R1-Zero and its replications: by removing the PRM and only assigning reward based on the symbolic criteria evaluated only for the final answer, they were actually able to get better performance.

Implementing PRMs in pipelines adds additional cost and friction to the development process, and may in fact lower performance when compared to skipping them entirely. R1-Zero shows they may not be worth the hassle--an important consideration given that they're also not as scalable of a technique, given that reward models tend to be brittle outside of the distributions that they were trained on.

\subsection{Using ITG}
Despite the fact that ITG techniques have been developed under a shroud of misunderstandings and anthropomorphizations, their popularity is unquestionable. We attribute this primarily to their effectiveness, especially on the sorts of measures that researchers have access to. Across many benchmarks, they *do* increase accuracy.

Previous works have often argued that these results are indicative of LLMs acquiring broad, general, and *novel* reasoning powers [CITE]. We will argue that the novelty of intermediate sequences that LLMs generate is often overstated, and that the existence of "aha" moments argues *against* this widely accepted view. Rather, we frame modern RL-driven ITG development as directly continuing previous approaches, whether prompt engineering focused or SFT, as we believe that all of these techniques fundamentally work by encouraging useful parts of the training distribution to surface.

One interesting question is of course how much recombination is necessary here! [CITE Ruiz] But that the level of recombination is at a very different level from what anthropomorphized analysis of the supposed semantic content of reasoning traces would push us towards--the model doesn't say "Wait, I should back up here" because it is pausing to think while outputting the stock phrase or because it is backtracking in its thinking, but because these are the sorts of sentences that are sufficiently high enough probability in the "reasoning" style of writing that it is replicating, which allow it to do "something like backtracking" NOTE this is a super vague point and I don't really know how I'm trying to phrase it here really... How do I distinguish between the semi-semantic content and the fact that the format it is forced into is really awkward and mirrors humans typing like they talk... (which also already for humans with the power to edit their text is nonsense!)
[NEED CITES here for how other people have framed why CoT is useful! especially super anthropomorphized versions!!]


\subsection{History of ITG}
% \begin{itemize}
%     \item ITG definition
%     \item How people have anthropomorphized CoT
%     \item CoT $\rightarrow$ ICL CoT $\rightarrow$ PRMs $\rightarrow$ RL-ITG
%     \item Papers confusing 'useful' and 'correct' internal tokens
%     \item People use ITG strategies because they often improve overall accuracies but CoT surfaces parts of the distribution - RL is no different.
% \end{itemize}

History of ITG in chronological order (with repeats from above, just diff organization)
\begin{itemize}
    \item Natural occurrences in math domains, presumably because of the amount of training data from educational webpages that provide step-by-step solutions
  \item Nye Scratchpads (required fine-tuning)
  \item Wei ICL CoT (with hand-crafted examples)
  \item Kojima zero-shot (domain general)
  \item the whole cottage industry of people doing this shit
  \item SFT on hand-crafted reasoning traces
  \item SFT on synthetically generated ones
\item SFT with filtering on self-generated ones
  \item Neural outcome reward models
  \item PRMs for trying to enforce "correctness" in traces
  \item R1-Zero style no PRM just symbolic answer verification

\item another important historical note is that it is unclear to what extent the observed increase in CoT's impact on performance is due to architectural, training, and scale advancements, and to what extent it originates from the data itself. It is entirely possible that the original data (sourced from a pre-LLM internet) contained many fewer examples of step-by-step derivations across domains, and that now pre-training corpora mass-scraped from anywhere are necessarily contaminated by traces that have naturally been filtered for quality by users prior to uploading. This speculation is beyond the scope of this paper, but hints towards a more holistic approach to evaluating LLM progress that takes into account the various unseen sources of contamination that naturally arise when LLMs are released at a rapid rate within an ecosystem that, through many opaque avenues, can feed information into models without even the trainers being explicitly aware. Another example: Pliny existing in the training data to the extent that jailbreaks are possible without even needing to do any real prompt hacking [CITE twitter, also see if there is any other stuff out there... also cite some contamination papers in general].
\begin{itemize}
    

\item Contamination is more complicated than just data. Arguably, researcher awareness of the types of problems that may be faced affects the sort of synthetic data that will be generated. We should move beyond the IID evaluation paradigm, as the more interesting thing is if you can still generalize outside of a given distribution.

\item Reasoning is about pushing the boundary outside of the data, not just interpolating. Hard to define. Move 37 is interesting because it came from basically nothing... just brute search compiled down over and over. My opinions on symbolic and neural needing to work together etc etc... NOTE move these bits out it's too far 
\end{itemize}
\end{itemize}
  \subsection{ Misc}
\begin{itemize}
\item Other random stuff
\begin{itemize}
  \item Expressiveness of CoT paper [CITE] and claims that it allows for all sorts of calculations that a vanilla Transformer model can't do in a single token--but it's unclear how this really differs from autoregression in general, as the boundary delimiting the two is fuzzy.
  \item Pause tokens, Let's think dot by dot [CITE] and other approaches that claim that the amount of computation {*in a single forward pass*} is meaningfully different as the input context fills up--which implies that the actual information content of the dots is mostly irrelevant (as it couldn't be that much...) NOTE figure out what the fuck is going on here
  \item Using CoTs as indicators of what the model is "thinking" and especially using these to analyze scheming capabilities and other safety concerns
  \end{itemize}
\end{itemize}
\subsection{ Faithful CoT}
\begin{itemize}
\item Faithful CoT papers
  \item interest in making CoTs actually "correct" not just lead to accuracy, with again the assumption that this will help with performance and be much more generalizable
  \item [CITE! What are the papers here anyway...]
  \item Intermediate tokens generated in response to "Let's think step by step" have long been known to be at least partly divorced from reality and be rather brittle.
  \item Faith and Fate analyzes intermediate generations to find that they have issues with cumulating error--if an early step is wrong within a pre-specified format, the entire chain can be disrupted. However, this analysis also makes clear that LLMs often (irregularly) pay attention to the "wrong" parts of the content in the context window, leading to generations where steps are suddenly corrected to what they should have been if a (potentially much) earlier mistake hadn't happened, or which make mistakes that should not have been made if they were only basing the next step on the calculations they were "claiming" to be doing--mistakes which, in isolation without the other context, the LLM never makes. Chain of Thoughtlessness corroborates this, especially in the arithmetic domain presented in that paper, where the particular (one-digit only) calculations are always solved correctly by LLMs at any temperature setting and at any size, but when they are required to do them in sequence, they suddenly start to make mistakes. NOTE check this with the prompts, maybe even rerun to have a cleaner domain version where there is no copying problem... Like the typo issue is much less interesting than a potential problem where an intermediate calculation is just completely done incorrectly! Though, even if the 100\% domains they were perfect at composition, they would still have composition issues in noisier domains. The issue of P(A,B) < P(A) *P(B), where P is probability of correctness.
\end{itemize}


==> sections/03-our_position.tex <==
\section{Our Position}
\begin{itemize}
\item Our position is that anthropomorphizing ITG is both an error in analysis that is sure to lead to incorrect conclusions and a red herring in implementation that leads to wasted time and resources.
\item In this section, we present our alternatives for how ITG *should* be analyzed and use these to motivate 
  \item ALT In this section we develop a principled framework for analyzing ITG and use it to argue against anthropomorphism and its downstream claims on both theoretical and practical grounds.

\item A frozen neural system can, in general, be analyzed using two factors: directly via the parametrized process that it uses to generate outputs, and teleologically via the pressures that led to the particular parameter set 
[CITE and check the McCoy teleological argument and where it comes from upstream! And briefly discuss where this kind of approach fails]
  \item We extend the approach from McCoy et al to a broader class of training regimes, and argue that the pre-training data likely explains a large portion of the surprising abilities witnessed even in R1-Zero style models--abilities which have previously been claimed or implied to somehow emerge due only to the power of reinforcement learning itself [CITE the RL does it all claims people make].
\item Process vs Pressure also directly maps onto the distinction between expressivity and learnability--just because a certain architecture or representation space is sufficiently expressive to capture a given algorithm or procedure does not mean that the associated learning algorithm will necessarily find that point let alone converge to it in the representation space. [CITE Alta and maybe briefly discuss how they approach this question... also CITE UAT and maybe some stuff following it up about how weak of a claim it really is]
  \item Previous work has looked at expressivity in a direct manner: given the transformer architecture (and perhaps some "scratch space") what class of algorithms could in principle be compiled into the network's weights? [CITE TC0 paper and brief sentence], with stronger claims made for models that implement CoT [CITE CoT expressivity paper].
\end{itemize}
\subsection{Pressures}
% \begin{itemize}
%     \item Human thought had totally different pressures
%     \item Possibility that more pre-train data has traces now, given CoT interest.
%     \item RL-ITG w/ KL is kept close to smoothed pre dist SO any innovations have to maintain the style, not contradict it. This is a pressure away from interpretability
%     \item Relation to the data is less clear for intermediate tokens
%     \item DRL sparse reward issues are overcome by soft-inductive bias of pretraining
%     \item CoT and LLMs "Failure to ignore"
% \end{itemize}
\begin{itemize}
    \item Another way to analyze the behavior and capabilities of an opaque system is the *teleological* approach, first applied to LLMs by McCoy et al. In this approach, we focus on the process that gave rise to the system, and use it to predict the sorts of capabilities it was most likely to give rise to/not give rise to. In the context of ITG, this may at first seem to be the RL post-training phase, but this is misleading. A system like R1-Zero first undergoes an extensive pre-training phase--a phase that not only uses the bulk of the total compute, but also results in a reference model that the RL phase is disincentivized from straying too far from.
    \item Therefore, analyzing the "novelty" or "emergence" of ITG behaviors that show up after the RL phase would--to be completely accurate--require access to the training data. If the behavior is already present in the training data, then RL isn't generating a totally novel sequence, and its ability to surface and rearrange already-present patterns efficiently tells us very little about this training regimes ability to move substantially beyond this data fast enough and robustly enough to beat other approaches.
  \item One argument, if we could use it, that would be very bullish for the possibility of getting general reasoning out of LLMs would be that, despite training on messy, web-scale, non-reasoning data, they nevertheless are pushed into producing coherent and human-like chains of thought with only the RL training phase. If true, this might point to a convergence towards some kinds of universal principles of good reasoning. However, this argument is fraught from the get-go.
    \item It is very likely the pre-training data has already been significantly contaminated over the last few years. Anecdotally speaking, since the release of Wei's 2022 CoT paper, there has been an explosion of interest in intermediate token sequences [cite number of papers talking about it, maybe GitHub presence somehow?] which show some evidence of or at least look like human-like reasoning processes. As these models are trained on massive scrapes of the internet, they've likely ingested a lot of this discussion, as well as the examples that tend to come with it--examples that are typically pre-filtered by the human discussing, and which therefore tend to not only be more often right in their answers, but also more correct or at least palatable as traces to the human posting them.
    \item [Cite llama contamination thing about AIME, contamination about AIME in general, any other cites on trace contamination]
    \item NOTE We can actually take this further, and look at the entire LLM training ecosystem as a set of processes guided by a set of competing actors and excited users. The extended game of whack-a-mole with some many people and resources involved that the goalposts can move faster than a given research group can blink... Find an example it doesn't work on and which gets sufficiently popular, it will end up in the pre-training data without anyone necessarily realizing it...
    \item The ITGs that we see from LRMs are often very verbose, winding sequences that locally seem to make sense, and which perhaps result in the right answer being output more often than otherwise, but which haven't been closely analyzed for overall coherence. Eyeballing a sample of them [include in the appendix some annotations or stats on repetition], they tend to be very repetitious [CHECK if this is true for both correct and incorrect ones!]. In other words, they are not particularly condensed or compressed. Thus, assuming that the model is learning some--potentially opaque and uninterpretable--algorithmic procedure that it is following in context, this procedure is far from compute-optimal. While optimal procedures for a given problem may be rather constrained, with few degrees of freedom, this is the opposite. The space of procedures that it could have learned that operate at this level of efficiency is quite large! The fact that the points that RL post-training finds in this space are at all human-like should actually be quite suspicious, and finger the pre-training data and resulting reference model as the culprit, rather than arguing for any sort of universality of human and machine cognition. It should also be a warning sign that anything truly novel will be novel not *because* it looks "human", but rather *despite* it. Reinforcement learning is capable of exploring new parts of the space, but it does so in ways fundamentally different from humans [cite or remove this sentence].
\item KL divergence keeps the model close to some smoothing of the pre-training data--any innovation has to maintain the style, not contradict it, which is a deliberate and necessarily deceptive step away from interpretability. (In fact, I'd even argue that we/safety people should be studying cases where this sort of deception arises--human-like reasoning would go in some direction, but the reward-hack has found a way through the space to just avoid that and get to the answer through some other approach anyway, especially since the pre-training in a sense argues against the data... TODO Easiest way to do this would be to train on wrong data!! Q/A pairs where the A is not correct (in some systematic way?) and the model picks up the arguments to systematically give this. Argue that this is true for e.g. data that is one way and then the distribution shifts over time, but the model is still arguing from its training. Could also do something like the answer is purely derived from the syntax... e.g. on integer questions and train to always output the number of vowels in the question or something similar
\item All of this brings up a significant problem: solid analysis requires access to the pre-training data and an understanding of the relationship between that data and the behaviors we see during ITG. Not only do we not have access to that data in most cases (Olmo family aside), but even if/when we do, the relationship is less clear in these cases than it is in vanilla pre-trained Transformer models without any form of SFT or RL post-training. Perhaps we can see the RL stage as re-weighting the pre-training data or preferring certain continuations (e.g. "Wait" a la s1 [Cite], which is itself a strong piece of evidence towards this position--an easy way to boost performance with just one token upweight, a KL-cheap method). This relationship can however be more complicated: the RL stage tunes the model to make KL-cheap choices in the space of language walks, but the particular walks that the final model prefers may be unpredictable and arise from more complicated statistical features than we can easily analyze. In other words, it may be easier to find what features are from the pre-training data than it is to discover and understand truly novel behavior.
\end{itemize}
\subsection{Process}

\begin{itemize}
    \item single forward pass argument--there is no distinction between the tokens that it outputs and the ones it is fed, it will react to them the same
  \item every pass is calculated by the same CPT
  \item No human-like continual thinking that proceeds in starts and bursts and stops, and which leads to irregularly time production of externalized language--a sharp contrast to the predictable and unvarying token output rate of language models [CITE both human stuff and the rate stuff for transformers]
  \item The only relationship between one forward pass and the next is the fact that it did come from the system, even if it doesn't matter that it did. From a pure expressivity perspective, we might consider each token as adding on a some additional information (as much as can be possibly encoded in a selection from the size of the vocabulary space), but if this is true, then how do we explain phenomena like the model outputting "hmm". 
    \item On one hand, perhaps it selected this token arbitrarily and it contains relevant information that will be accessible in the next forward pass computation but is opaque to us--which doesn't explain at all why the specific human-like token, and, worse, doesn't give us any insight into what information was encoded and how it will be used.
    \item On the other, perhaps--like the way humans use it, a delaying tactic--the token *doesn't* contain information that will be important to the next computation, in which case, during the next forward pass, the model will be doing the same full set of computations without any relevant progress having been made. In this case, we are still left with the need to explain why the token is there, but it also is not being used for the same underlying reasons that a human would. NOTE: this bit is all loopy and repetitive. Fix later
    \item Even stronger is the case of the finger-counting LLM [CITE tweet], where intermediate tokens claim that there is a separate process occurring which we also know is impossible to actually be occurring, as language models do not have bodies let alone fingers to do such counting on. It is all style, no substance. The standard we apply to obvious misrepresentations of physicality should also apply to the same kind of misrepresentations of computation capability!
  \item in general, ITG allows only for myopic changes, eventually creating an augmented prompt for the model to ingest that is hopefully more likely to give the right answer. There is no underlying world model that is changed at each token, maintained for the next, and changed again. Instead any internal representations must be reconstructed from scratch at each pass [CITE or at least find some backup to discuss]
\item If any anthropomorphization were accurate here, it would have to be closer to a case even more severe than 7-second Clive looking at his diary and seeing it for the very first time, but instead of crossing out the previous entry as a falsification of his writing, merrily going along with what is already writing before having to start anew at the next word [CITE Clive Wearing, also check transformers are fully discrete in this manner]

\item Learning local post-fixes *could* make sense
  \item entirely possible that the model learns that when the current context ends in a certain way, it should always be completed in some particular manner
  \item This, in aggregate, would be approximately rule-based reasoning, and while it still wouldn't warrant anthropomorphizing the process, it could then be interpreted as executing a sort of fuzzy rule-based inductive reasoning. However, in practice, this has been found to be somewhat brittle, even for problems that--in isolation--the model can solve with perfect accuracy [CITE F\&F, CoTlessness]. NOTE: am I repeating from the background section here? Where should this discussion live (or die)?
\item In general, approaches that recognize the static, frozen nature of the autoregressive network have promise for providing clearer analysis. 

\item information-theoretic approach
\item CITE need some sources on the functions of Hmm and other delaying sounds in actual humans, so that we can argue that these functions CANNOT be the same for the LLM!
\item The function of these human-seeming token sequences that "naturally emerge" during the RL training is thus fundamentally different from their function in humans. To properly understand where they come from and why they are replicated, we argue that we will need to look at the pressures that gave rise to the model.
\item However, we do also have evidence from Pause Tokens and Think Dot by Dot [CITE] that the amount of context fed to the model itself is an important predictor of performance--which can be explained by [CHECK CITE] the increase in computation made available. This can only be explained with reference to the architecture itself, and--in fact--analyzing the model from the perspective of the architecture gives strong hints that lead us to look *in the right places*. 

\item NOTE: reorganize this, especially with the info-theory stuff scattered. Need good citations to really anchor what's being argued here and to arrange it usefully.
\end{itemize}


==> sections/04-benefits.tex <==
\section{Benefits of our position}
% \subsection{Interpretation and Evaluation}
% \begin{itemize}
%     \item Predictability and safety
%     \item In general, reasoning ability is how far can you go beyond the distribution with only a little new data
%     \item (Safety) o1 Scheming Paper
%     \item (Safety) Dangerous to anthropomorphize as ascribing goal-directedness with an assumed (but wrong) goal will be at best misleading.
%     \item human-looking not human-like
%     \item Intervening at the token level in ITGs can be an interpretability tool
%     \item Rising cost as an argument against human-likeness
%     \item Failure modes of RL-ITG will be similar to RLHF and are best understood from data (e.g. Pliny hack)
% \end{itemize}
% \subsection{Implementation and advancements}
% \begin{itemize}
%     \item Dont delude ourselves about whether human-like is for performance or readability
%     \item SUttons Bitter Lesson: Simple archs that scale win. Understanding relationship to data and how far it allows for further training is key to rapid progress.
%     \item Sound verifier$>$hackable outcome models (Sasha rush tweet ;))
%     \item teleological pressure vs process arg
%     \item Distinguishing 'hard to verify' from 'no ground truth' domains - and argue that rapid steerability matters more in creative writing like tasks
% \end{itemize}

\subsection{Why? Interpretation and Evaluation}

\begin{itemize}
\item By disentangling the confused concepts of "human-looking" token sequences and "human-like" reasoning,

\item Safety and predictability
\begin{itemize}
  \item scheming paper CITE
  \item In general, we believe that safety work that starts from the premise [CITE CHECK THAT THIS IS EVEN RELEVANT, LOOK AT SOME PAPERS THAT CLAIM THIS-ish] that we can deduce an LLM's actual goal from what sorts of intermediate tokens it produces can be very misleading. Even assuming that modeling the inference process as goal-optimizing even makes sense [maybe cite Xuan beyond prefs??], if we deduce the wrong goal because we use intuitions that are applicable to the only other language users that produce these kinds of sequences (aka humans) but which fall apart when applied to these systems, this sort of analysis will be at best misleading. We think it is important to find actual examples of deception, which will likely be much more complicated in higher-compute and more advanced future systems, and less pre-training data dependent in the sorts of systems for which long-term safety and robustness actually matter. 
  \begin{itemize}
    \item Avoid boy who cried wolf situations
    \item Avoid wasting time on fleeting failure modes that are unlikely to generalize or be relevant in the same ways in the future, in the systems for which safety and steerability will matter much more
  \end{itemize}
\end{itemize}
\todo{specify the safety stuff a lot more thoroughly. Be way clearer here! Look into the citations}

\item Reasoning ability is how far you can generalize beyond the dataset [CITE Chollet, other relevant stuff]

\item By analyzing ITGs from the viewpoints we offer and rejecting anthropomorphization (except where it is warranted--in particular the pre-training data \textit{is} human-generated and must be treated as such, and must also be assumed to be the most likely source of human-like behavior), we believe more productive approaches can be derived:
  \item examples: 
  \begin{itemize}
    \item intervening at the token level in ITGs as an interpretability tool
    \item ablating R1-Zero style systems. Yes it works when we do the expected thing, but what about training with differently pre-trained models, ideally without any traces in the original data, or by training it to contradict the training data?
    \item Realizing that capturing more of the frontier, in a generalizable way, may require further hacks to the sorts of training data that is fed to the model. Also a further focus on continual learning/active learning techniques [CITE?? what's this work look like]
    \item throwing away the SFT stages and PRM approaches--something R1-Zero already did--or realizing that they are only there because we *want\item the trace to \textit{seem} human-like for end-users.
    \begin{itemize}
      \item if we keep them, don't kid ourselves! And don't trust them to somehow do away with the long-running hallucination problem that has plagued these models since they first started being trained. 
    \end{itemize}
    \item Pre-training over non-linguistic spaces or allowing further deviation to let the model pick up weirder and less comprehensible ITGs, since we already believe that their relation to human reasoning or legibility is tenuous and at best just reduces the search space (potentially too far) to a smoothed space of walks through pre-training language.
    \begin{itemize}
      \item another view is that the model is both (fuzzy) language specification and compiler/executor... we train it to find a find a ~linear/~feedforward [cite what would this mean... whats the class] coding language that better solves the problems it is RL'd on.
    \end{itemize}
  \end{itemize}
  \item Our perspective also provides hints for how we should approach a very important question that has till now only been answered in the vaguest terms: What properties are necessary for an underlying model to be able to support ITG-RL post-training? Previous discussions [cite] have only really mentioned that previously similar techniques didn't work because previous models weren't "good enough", conflating model size and amount of training data, but not digging any deeper into which features of the model architecture/scale or data are relevant and can be modified to better support RL training pipelines. We believe that this is an open question, but that there may be insight in looking into what data the underlying model has been trained on, and trying to predict the relationships between features of that data and predicted features of the processes necessary to solve pre-selected classes of new problems.
  \begin{itemize}
    \item NOTE maybe also connect this to the large over-parametrized models capture "simpler/more generalizable" high-dimensional descriptions [see the strangelove paper again on that front]
   \end{itemize}
  
\item We also will get more plausible and well-articulated arguments for things like the "aha" moment rather than breathless hype [CITE wasn't someone already saying on twitter that they were rejecting the aha moment on data grounds?]

\item a return to seeing the data as primary! And to being able to separate the additional progress given by RL from what it is surfacing.

\item also a push towards understanding why so much repetition arises, even though from an efficient computation perspective, we should expect a good learner to teach itself short ITGs not only because of resource-rationality [CITE] but because of the reusability of short concepts leading to useful generalizations [CITE library work]

\item Q: is there a way of seeing a lot of the repetitious behavior of R1 as really being in-context multiple CoT generation and then averaging... aka "emergent" self-consistency? This could actually be something a little beyond the training data, as it would be using the summarizing capabilities to extract the common chains and then using those to make the final answer decision...

\item Q: Can we actually use the convergent rate of SFT to characterize the "learnability" of techniques? Aka to characterize the chance that RL will surface a certain behavior. What I mean by this is: say that we want to know if some behavior is important to solving a problem (and is also visible in R1 traces), then we could construct two datasets: one that is generated by the model of examples with perhaps permutations and one that is just synthetic and looks different but does the "same reasoning". We should expect a difference in learnability between these, favoring the model's version, if we train the base model with SFT on these traces. 
\begin{itemize}
\item Q: the more interesting version is the question of, given a reasoning behavior, does there exist some version of it already latent in the model, which would be easier to SFT. And more importantly for applications, can we search for it somehow?
\item Q: very related to the general question of if locally probable things retain that local probability in other cases... like it could be that there's a really specific set of conditions in which it is high prob, but not in any other, in particular not in the cold-start, empty-prompt case! This is especially obvious in DeepSeek MoE models, but probably also true given some level of disentanglement in any transformer architecture...
\end{itemize}
\end{itemize}

\subsection {Why? Implementation and Advancement}
\begin{itemize}

\item We also believe that moving away from unwarranted anthropomorphism is beneficial for building better models in the future and accelerating the pace of the development of not just LLM reasoners in general, but specifically of more interpretable or at least less deceptively interpretable models.

\item Don't delude ourselves about whether human-legibility of ITGs is for performance or just for end-users! If we toss out the latter concern, we can experiment with much weirder, simpler approaches. Instead of, for example, SFTing on human-written or synthetically generated traces, we could just enforce simple locality constraints or other pressures towards generality that may not have obvious relations back to human data

\item The teleological or process/pressures perspective provides direct guidance on where to improve these models:
\begin{itemize}
  \item Process constraints indicate that perhaps we should move past the raw autoregressive paradigm towards either modified architectures [cite and discuss Coconut + the new paper with the recurrent block + etc] that dispense entirely with attempts to be human interpretable, whether because they move into continuous spaces or because they ??? is there a second option; or towards compound systems, such as those that incorporate things like MCTS [cite], use static programmatic components to insert additional intermediate or tool-call-response tokens [cite s1, dot by dot, etc], or verify or produce answers or substeps through formal methods [cite modulo, LLM+P, all that stuff].
  \item The pressure perspective argues for being able to modify and induce interesting behaviors via changing the pressures that give rise to the final model.
  \begin{itemize}
    \item From R1-Zero, we also see that sound verifiers seem to do better than hackable reward models, pointing at the need for pressures that can't be "cheated", that is, actually capture the behavior that we want. However, even with sound verifiers, we should remain wary of what sort of Q/A data we are RL training on, as what it doesn't capture still leaves open significant holes! NOTE in particular this may argue for adversarial Q/A generation, where we pair a sound verifier with a problem generator--allowing us to search for problems that still trip up the model and focus our training efforts on those [e.g. could cite extensions of the active learning of let's verify step by step]. Even with this, we will only ever be at all confident that those problems captured by our set of generator/verifier pairs are solvable by our models... and its unclear how they will generalize beyond these domains, or even how well they will interpolate between them
   \end{itemize}
\end{itemize}
\item In future applications, we will want models that generalize beyond their RL'd data, but that also can deal with complex, differing situations. In domains with one right answer, like integer solution math problems (e.g. AIME), the exact process used to reach the answer is much less important than the fact that the answer is right. Therefore, strong biases to solve things in particular ways and output a lot of tokens that the final answer will condition on (and thus potentially [CITE? CHECK? ARGUE???] be dragged back into the space of typical outputs for the model) are entirely fine. This extends to any answer that can be formally checked, such as Lean proofs, but it doesn't extend to domains like creative writing or informal proofs, where the humans preferences or needs are crucial constraints on the sorts of output that should be generated. Current approaches do not seem to take into account this difference in how steerable the model should be across classes of queries, instead trusting that the "human-like" nature of chains of thoughts will capture this automatically. [CITE and verify] We see no reason to believe this a prior, and encourage more explicit research into solving this problem.

\item An Endemic Misapplication of Sutton's Bitter Lesson
\begin{itemize}
  \item Simple architectures that scale, win
  \item But the architecture and training procedures we're seeing in these models is only simple in an illusory sense: The pre-training process, the base model architecture, and the idea of RL training are all simple. BUT the amount of data required for performance is huge, and this data is run through opaque, generally under-reported [CITE AND CHECK OLMO THOUGH] data filtration and cleaning processes which seem to be crucial to the levels of performance that we do see.
  \item We have no clear understanding of how much and what kind (and how much pre-processing is necessary) of data is necessary to get the RL-ITG results we are currently seeing. If performance cannot scale beyond the data, then we will continue to be limited by the amount of high-quality data that we can produce. In the worst case, this limits the regime to the slower cycle of model release, public use and internet contamination, large web-scale scrapes, and new model training.
  \begin{itemize}
    \item This view does open up one useful interpretation: with some effort, we can convert compute into synthetic data. This still doesn't uncap scaling, as specifying synthetic data generators is still in the hands of researchers and engineers, but it does allow us to move up a further level of abstraction: from direct feature engineering to data curation and creation for automatic feature engineering to partial algorithm specification for automatic data creation.
    \item Also opens up the possibility of train-time modulo and verifier synthesis.
    \item \textit{Do I keep this?} Or of ways to more carefully move the reference model around or inject additional features/patterns into it that can then be learned to be rearranged properly by RL
  \end{itemize}
\end{itemize}
\end{itemize}

==> sections/05-openq.tex <==
\section{Open Questions}
\begin{itemize}
    \item Can we tell if a pretrained model has relevant latent knowledge or is close enough w/o RL?
    \item What is the tradeoff between model size/quality and is RL necessary?
    \item How well does RL-ITG generalize to other domains esp with those w/o easy verification
    \item Value of legible CoTs
    \item R.D: Self generation of problems in a verifier framework--true self-play within some limit
    \item R.D. General verifiable domains 
\end{itemize}


==> sections/06-altviews.tex <==
\section{Alternative Viewpoints}
\begin{itemize}
    \item For convergence or/and performance ITGs must be semantic
    \item Semantics will emerge eventually
    \item Stronger additional fuzzy semantics do directly and predictably help (R1-zero vs R1)
\end{itemize}

Papers that have anthropomorphized COT,
\begin{itemize}
    \item COT
    \item Kojima COT 
    \item Verify COT
    \item Researchers pushing for correctness of reasoning chains - SelfCheck, AutoRace
    \item 
\end{itemize}

==> sections/07-concl.tex <==
\section{Conclusion}

==> tts-pt-minipage.tex <==
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{images/tts_figure1.png}
  \caption{Test-time scaling}
  \label{fig:tts}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{images/pt.png}
    \caption{Post-training}
 % \captionof{figure}{Another figure}
  \label{fig:post}
\end{subfigure}
\caption{Post-Training and Test-Time Scaling approaches for teasing out reasoning}
\end{figure}


\begin{figure}
\centering
\begin{minipage}{.5\linewidth}
  \centering
  \includegraphics[width=.4\linewidth]{images/tts_figure1.png}
  \captionof{figure}{Test-time scaling approaches for teasing out reasoning}
  \label{fig:tts}
\end{minipage}%
\begin{minipage}{.5\linewidth}
  \centering
  \includegraphics[width=.4\linewidth]{images/pt.png}
    \captionof{figure}{Post-training Approaches for teasing out reasoning}
 % \captionof{figure}{Another figure}
  \label{fig:post}
\end{minipage}
\end{figure}

